Regular Matroids with Graphic Cocircuits

We introduce the notion of graphic cocircuits and show that a large class of regular matroids with graphic cocircuits belongs to the class of signed-graphic matroids. Moreover, we provide an algorithm which determines whether a cographic matroid with graphic cocircuits is signed-graphic or not.

==> eptcsdata.tex <==
\providecommand{\event}{E. Markakis, I. Milis (Eds.): 4th Athens Colloquium\\ 
on Algorithms and Complexity (ACAC 2009)}
\providecommand{\volume}{4}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{29}
\providecommand{\eid}{4}

